Permissionless and Asynchronous Asset Transfer [Technical Report]

Most modern asset transfer systems use consensus to maintain a totally ordered chain of transactions. It was recently shown that consensus is not always necessary for implementing asset transfer. More efficient, asynchronous solutions can be built using reliable broadcast instead of consensus. This approach has been originally used in the closed (permissioned) setting. In this paper, we extend it to the open (permissionless) environment. We present Pastro, a permissionless and asynchronous asset-transfer implementation, in which quorum systems, traditionally used in reliable broadcast, are replaced with a weighted Proof-of-Stake mechanism. Pastro tolerates a dynamic adversary that is able to adaptively corrupt participants based on the assets owned by them.

==> LA-PoS/Abstractions.tex <==
% In this section we define two abstractions that serve as the main building blocks of our asset-transfer implementation. 
% \\

% \myparagraph{Transaction Validation Protocol.} The \emph{Transaction Validation Protocol} (TVP) is an abstraction through which transactions pass and receive certificates of their validity. 
% This abstraction can be considered as a filter for submitted transactions, that passes only the ones that don't conflict with each other.

% Transaction $tx = (p, \tau, D) \in \tT$ is called \textit{verifiable} iff it is verifiable in terms of verifying function $\code{VerifySender}(tx, \sigma_{tx})$. Here, $\sigma_{tx} \in \Sigma_{\tT}$ is a certificate that proofs that a valid transaction $tx$ was actually being issued by a member $p$.
% It's natural to think of transaction certificates as of their digital signatures. 
% We assume that adversary is unable to compute a valid certificate for a transaction that it didn't submit itself: if $p$ didn't submit transaction $tx$ to the protocol, then any correct process returns $\false$ from $\code{VerifySender}(tx, \sigma_{tx})$ for any potentially received $\sigma_{tx}$.

% The Transaction Validation Protocol abstraction exports one operation and one function:
% \begin{itemize}
%     \item Operation $\code{Validate}(tx, \sigma_{tx})$ returns a pair $\langle txs, \sigma_{txs} \rangle$, 
%     where $tx \in \tT$ is a verifiable transaction, $\sigma_{tx} \in \Sigma_{\tT}$ is a valid certificate for transaction $tx$,
%     $txs \in 2^{\tT}$ is a verifiable (output) transaction set, and $\sigma_{txs} \in \Sigma_{2^{\tT}}$ is a valid certificate for a transaction set $txs$.
%     \item Function $\code{VerifyTransactionSet}(txs, \sigma_{txs})$ returns $\true$ if $\sigma_{txs}$ is a valid certificate for output transaction set $txs$, else returns \textit{false}.
% \end{itemize}
% Transaction set $txs$ is called \emph{verifiable} iff it is verifiable in terms of verifying function $\code{VerifyTansactionSet}$.

% Implementation of Transaction Validation Protocol should satisfy the following properties: 
% \begin{itemize}
%     \item \emph{TVP-Verifiability}: If $\code{Validate}(\dots)$ returns $\langle txs, \sigma_{txs} \rangle$ to a correct process, then\\ 
%     $\code{VerifyTransactionSet}(txs, \sigma_{txs}) = \true$;
%     \item \emph{TVP-Inclusion}:  If $\code{Validate}(tx, \sigma_{tx})$ returns $\langle txs, \sigma_{txs} \rangle$ to a correct process, then $tx \in txs$;
%   \item \emph{TVP-Validity}: Every returned verifiable transaction set contains only verifiable transactions and all transactions from all returned verifiable transaction sets don't conflict with each other; 
%     % \item \emph{TVP-Liveness}: If the number of protocol members is finite
%     % and a forever-correct process invokes $\code{Validate}(t, \sigma_t)$, then some forever-correct process eventually returns  $\langle trs, \sigma_{trs} \rangle$, where $t \in trs$.
% \end{itemize}
% We also introduce the following condition for dynamicity: \emph{all properties must be met even if configuration of the system changes}. 
% We say that an instance of some TVP implementation is \textit{dynamic} if it meets the above condition.
% \\

% \myparagraph{Byzantine Lattice Agreement.} \emph{Byzantine Lattice Agreement} (BLA) is a Lattice Agreement~\citep{gla} that tolerates Byzantine failures of processes.
% This abstraction is parameterized by a join semi-lattice $\Lat$, and a boolean function $\code{VerifyInputValue}: \Lat \times \Sigma_{\Lat} \rightarrow \text{Bool}$.

% An input value $v \in \Lat$ is called \emph{verifiable} iff it is verifiable in terms of function \code{VerifyInputValue}.
% Unlike the Transaction Validation Protocol, where verifying function (\code{ValidSender}) is fixed, BLA allows to specify this function depending on the needs. 

% Byzantine Lattice Agreement exports one operation and one function:
% \begin{itemize}
%     \item Operation $\code{Propose}(v, \sigma_v)$ returns a pair $\langle w, \sigma_{w} \rangle$, 
%     where $v, w \in \Lat$ , $\sigma_v \in \Sigma_{\Lat}$  is a valid certificate for input value  $v$, $\sigma_{w} \in \Sigma_{\Lat}$ is a valid certificate for output value $w$;
%     \item Function $\code{VerifyOutputValue}(w, \sigma_{w})$ returns $\true$ if $\sigma_{w}$ is a valid certificate for output value $w$, else returns \textit{false}.
% \end{itemize}
% Output value $w$ is called \emph{verifiable} iff it is verifiable in terms of verifying function $\code{VerifyOutputValue}$.

% Implementation of Byzantine Lattice Agreement should satisfy the following properties:
% \begin{itemize}
%     \item \emph{BLA-Validity}: Every verifiable output value $w$ is a join of some set of verifiable input~values;
%     \item \emph{BLA-Verifiability}: If $\code{Propose}(\dots)$ returns $\langle w, \sigma_{w} \rangle$ to a correct process, then \\ $\code{VerfyOutputValue}(w, \sigma_w) = \true$;
%     \item \emph{BLA-Inclusion}: If $\code{Propose}(v, \sigma_v)$ returns $\langle w, \sigma_w \rangle$, then $v \sqsubseteq w$;
%     \item \emph{BLA-Comparability}: All verifiable output values are comparable.
%     % \item \emph{BLA-Liveness}: If the total number of members is finite
%     % and a forever-correct process invokes $\code{Propose}(v, \sigma_v)$, then some forever-correct process eventually returns  $\langle w, \sigma_{w} \rangle$, where $v \sqsubseteq w$.
% \end{itemize}
% Similarly to Transaction Validation Protocol, we impose a dynamicity condition: \emph{all properties must be met even if configuration of the system changes}, an instance of some BLA implementation is said to be \textit{dynamic} if it meets this condition.


% With the help of Byzantine Lattice Agreement instance we can produce configurations that are comparable (i.e., all transactions sets will be related by the containment $\subseteq$). 
% In addition, using another BLA instance, that is parametrized with set of configurations as a lattice, we can obtain sets of configurations, that are related by the containment. 
% If only comparable configurations are allowed in input sets (e.g., such requirement might be established via verifying function), then all output sets of configurations are related by the containment and configurations in this sets are comparable. We can consider these sets as sequences of ordered configurations. 
% Such sets are called \emph{histories} and were presented in recent paper on asynchronous reconfigurations~\citep{bla}.
% Histories allow to access only $O(n)$ configurations, when $n$ configurations are concurrently proposed. 
% History is called \emph{verifiable} iff it's verifiable in terms of function $\code{VerifyHistory}(h, \sigma_h)$.

% \textbf{Remark}. For simplicity, we don't require liveness property neither in Transaction Validation Protocol, nor in Byzantine Lattice Agreement. 
% We use them only as building blocks for another abstraction that solves asset-transfer problem, and guarantee liveness only for that ``bigger'' abstraction. \\


==> LA-PoS/crashes/Algo.tex <==

\myparagraph{Overview.}
%
The algorithm is specified by the pseudocode of Figure~\ref{fig:cla}. Note that we assume that all procedures
(including sub-calls to the \emph{updateState} procedure) are executed \emph{sequentially} until they terminate 
or get interrupted by the wait condition in line~\ref{line:cla:wait}.

We say that a state is \emph{committed} if a process broadcasted it in line~\ref{line:cla:bcast}. 
In the algorithm, every process (client or server)~$p$ maintains a \emph{configuration} variable $c_p\in\cC$ 
storing its local estimate of the greatest committed configuration state,  initialized to the initial element of the lattice $C_0$. 
Note that all learnt states are committed (possibly indirectly by another process), 
but a process may fail before learning its committed state. 
%
Every process $p$ also maintains $T_p$, the set of \emph{active} \emph{input} configuration states, i.e., 
input configuration states that are not superseded by the committed state estimate~$c_p$.  


To propose $\mathit{proposedConfig}$, client $p$ updates its local variables through the \emph{updateState} procedure 
using its input configuration state and ${proposedConfig}$ (line~\ref{line:cla:initState}).
Clients then enter a while loop where they send \emph{requests} associated with their current sequence number 
$\textit{seq}_p$ and containing the tuple $(c_p,T_p)$, to all the replicas.
Then, they wait until either (1)~they get interrupted by discovering a greater committed configuration 
through the underlying reliable broadcast, or (2)~for each possible join of input configurations with the commit estimate configuration, 
a quorum of its replicas responded with messages of the type $\langle (\textit{resp}, \textit{seq}_p), (c,S_C) \rangle$, 
where~$(c, S_C)$ corresponds to the replica updated values of its tuple $(c_p,T_p)$ (lines~\ref{line:cla:send}--\ref{line:cla:wait}).

Whenever a process (client or replica) $p$ receives a new request, response or broadcast of the type 
$\langle \textit{msgType},(c,S_C)\rangle$, it updates its commit estimate and object candidate 
by joining its current values with the one received in the message. It also 
merges its set of input configurations $T_p$ with the received input configurations, 
but the values superseded by the updated commit estimate are trimmed off $T_p$ 
(lines~\ref{line:cla:newCommit}--\ref{line:cla:newConfs}).
Replicas send a response containing the updated tuple $(c_p,T_p)$
to the sender of the request (line~\ref{line:cla:sendback}). 

If responses from quorums of all queried configurations are received and no
response contained a \emph{new}, not yet known, input configuration, 
then the join of the commit estimate configuration with all input configurations 
$\bigsqcup^\cC (\{c_p\}\cup T_p)$ 
is broadcasted and returned as the new learnt state (line~\ref{line:cla:return}). 
Otherwise, clients proceed to a new round. 


%
\begin{figure}[!]
\hrule \vspace{1mm}
 {\small
\setcounter{linenumber}{0}
\begin{tabbing}
 bbbb\=bbbb\=bbbb\=bbbb\=bbbb\=bbbb\=bbbb\=bbbb \=  \kill
\textbf{Local variables:} \\
$\textit{seq}_p$ : Int = $0$\ \ \ \ \commentline{The number of issued requests}\\
$c_p : \cC$ = $C_0$\ \ \ \ \ \ \   \commentline{The last learnt configuration}\\
$T_p : Set\langle\cC\rangle$ = $\emptyset$\commentline{The set of proposed configuration states}\\
\\
%
%
\textbf{fun} propose$(\text{proposedConfig}: \cC): \cC$\\
\nnll\label{line:cla:initState}\> updateState$(c_p,\{\text{proposedConfig}\})$\\
\nnll\label{line:cla:while}\> \textbf{while} \textit{true} \textbf{do}\\
\nnll\label{line:cla:seqNum}\>\> $\textit{seq}_p \leftarrow \textit{seq}_p+1$\\
\nnll\label{line:cla:refCommit}\>\> \textbf{let} oldCommit =  $c_p$.\text{copy}$()$ \\
\nnll\label{line:cla:refCandidates}\>\> \textbf{let} oldCandidates = $T_p$.\text{copy}$()$ \\
\nnll\label{line:cla:queriedConfs}\>\> \textbf{let} $V = \{\bigsqcup^\cC (\{c_p\}\cup S)~|~S\subseteq T_p\}$\commentline{Queried configurations}\\
\nnll\label{line:cla:send}\>\> \textbf{broadcast} $\langle (\textit{REQ},
\textit{seq}_p),(c_p,T_p)\rangle$\\
\nnll\label{line:cla:wait}\>\> \textbf{wait until} $\text{oldCommit} \neq c_p$ \textbf{or} 
$\forall u \in V$, received responses of the type  \\
\>\>\>\>\>  $\langle (\textit{RESP},\textit{seq}_p),\_ \rangle$ from some $Q\in\textit{quorums}(u)$\\
\nnll\label{line:cla:noInterrupt}\>\> \textbf{if}  $\text{oldCommit}=c_p$ \textbf{and} $\text{oldCandidates} = T_p$ \textbf{then}  \commentline{Stable configurations}\\
\nnll\label{line:cla:bcast}\>\>\> \textbf{broadcast} $\langle \textit{COMMIT},((\bigsqcup^\cC (\{c_p\} \cup T_p),\emptyset) \rangle$\\
\nnll\label{line:cla:return}\>\>\> \textbf{return} $(\bigsqcup^\cC (\{c_p\}\cup T_p))$\\ 
\nnll\label{line:cla:otherCommit}\>\> \textbf{if} $\text{proposedConfig} \sqsubseteq 
c_p $ \textbf{then} \\
\nnll\label{line:cla:otherCommitReturn}\>\>\> \textbf{return} $c_p$ \\
\\
%
%
\textbf{private fun} updateState$(c: \cC,\ S_C: \text{Set}\langle\cC\rangle): \text{void}$ \\
\nnll\label{line:cla:newCommit}\> $c_p \leftarrow c_p\sqcup c$\\
\nnll\label{line:cla:newConfs}\> $T_p \leftarrow \{u\in (T_p\cup S_C)~|~u\not\sqsubseteq^\cC c_p \}$ \\
\\
%
%
\textbf{upon} receive$(\langle \text{msgType},~\text{msgContent} \rangle \ q: \text{Sender}): \text{void}$ \\
\nnll\label{line:cla:mergeReceived}\> updateState(msgContent) \\
\nnll\label{line:cla:sendback}\> \textbf{if} $\text{msgType}=(\textit{REQ},\textit{seq}) $ \textbf{then} \textbf{send} $\langle (\textit{RESP},\textit{seq}),(c_p,T_p)\rangle$ to $q$\\ 
\\

\end{tabbing}
}
\vspace{-1.5mm}
 \hrule
\caption{Universal reconfiguration construction: code for process $p$.}

\label{fig:cla}
\end{figure}

\myparagraph{Correctness.}
Now, we will show that algorithm specified in Figure~\ref{fig:cla} satisfies the consistency, validity and reconfigurable liveness properties.

%
\begin{theorem}
\label{thm:consistency}
The algorithm in Figure~\ref{fig:cla} satisfies the consistency property.
\end{theorem}
\begin{proof}
It is direct corollary of Theorem 5.1 from ~\cite{rla}.
\end{proof}

%
\begin{theorem}
\label{thm:validity}
The algorithm in Figure~\ref{fig:cla} satisfies the validity property.
\end{theorem}
\begin{proof}
It is direct corollary of Theorem 5.2 from ~\cite{rla}.
\end{proof}

\begin{lemma}
\label{lm:progres}
In every execution with at least one invocation of $\textit{propose}(c)$, some process $p$ broadcasts a commit message at line \ref{line:cla:bcast}. 
\end{lemma}
\begin{proof}
We will prove this fact by contradiction. 
Let us assume that there is no such process, that invokes  $\textit{propose}(c)$ and broadcasts a commit message. 
As the number of members is limited by some $n$, then number of $\textit{propose}()$ invocations is limited by $n$ as well.
In this case, all processes $p_i$ that invoke $\textit{propose}()$ should eventually have equal sets of proposed configuration states $T_{p_i}$.
It means that eventually some process $p$ should pass the test at line \ref{line:cla:noInterrupt} 
and broadcast a commit message at line \ref{line:cla:bcast}. Contradiction.
\end{proof}

\begin{lemma}
\label{lm:sysprogres}
The algorithm in Figure~\ref{fig:cla} guarantees system-wide progress. 
\end{lemma}
\begin{proof}
By lemma \ref{lm:progres} at least one process broadcast a commit message 
during the execution. By applying proof of the lemma recursively we obtain the desired property.
\end{proof}
\begin{theorem}
\label{thm:liveness}
The algorithm in Figure~\ref{fig:cla} satisfies the CLA-Liveness property.
\end{theorem}
\begin{proof}
Let's consider a configuration $C_p$, proposed by the process $p$. 
We show that this configuration is eventually committed, and hence, operation $\textit{propose}(C_p)$ invoked by process $p$ eventually returns.\\
Note that $\textit{propose}(C_p)$ is in progress if process $p_i$ either learns that some other process committed a greater configuration (w.r.t. $\sqsubseteq$) or set of 
proposed configurations has changed (line \ref{line:cla:noInterrupt}), 
and no other process has committed a configuration $C: C_p \sqsubseteq C$ (line \ref{line:cla:otherCommitReturn}).
Recall that we only consider executions where $\forall C \in \cC: |\textit{members}(C)| \leq n$. Taking this 
into account and the definition of $members(C)$, we obtain following: there exists a configuration $C_{n_0}$ 
such that $\forall C \in \cC: \textit{members}(C) \subseteq \textit{members}(C_{n_0})$. Hence, after
configuration $C_n$ (such that $C_{n_0} \sqsubseteq C_n)$ is committed and learnt by $p$, 
all correct processes will eventually receive a message 
$m = \langle(REQ, \_), (\_, T_p)\rangle$ (where $C_p \in T_p$) and 
add $C_p$ to their local proposed configuration states (line \ref{line:cla:mergeReceived}). 
Hence, any process that broadcasts a commit message after 
receiving message $m$ will also commit a configuration $C_p$. By lemma \ref{lm:sysprogres} such process must exist.

\end{proof}
  
 
\begin{figure}
\hrule \vspace{1mm}
 {\small
\setcounter{linenumber}{0}
\begin{tabbing}
 bbbb\=bbbb\=bbbb\=bbbb\=bbbb\=bbbb\=bbbb\=bbbb \=  \kill
\textbf{Shared:}  $\textit{CLA}$, configuration lattice agreement\\
%\\
\textbf{Local variables:}\\
\> $C_p :\cC = C_0$  \commentline{The last learnt configuration state}\\
%\\
\\
\textbf{upon invocation of} $a\in A^{\cC}$ \\
\nnll\label{line:ladt:checks}\> \textbf{if} \textbf{not} $\textit{isValid}(C_p, a)$ \textbf{then} \commentline{Application specific checks (optional) } \\
\nnll\label{line:ladt:invalidreturn}\>\> \textbf{return} \\
\nnll\label{line:ladt:rinvoke}\> $C_p :=\textit{CLA}.\textit{propose}(\tau^{\cC}(C_p, a))$\\
\nnll\label{line:ladt:rreturn}\> \textbf{return} $\delta^{\cC}(C_p,a)$
\end{tabbing}
}
\vspace{-1.5mm}
 \hrule
\caption{Interval-linearizable implementation of L-ADT
 $L=L^{\cC}$: code for process $p$.}

\label{fig:ladt}
\end{figure}

\begin{theorem}
\label{thm:validity}
The algorithm in Figure~\ref{fig:ladt} is a reconfigurable implementation of a L-ADT.
\end{theorem}
\begin{proof}
TODO \\

\end{proof}


==> LA-PoS/crashes/Cryptocurrency.tex <==
In this section, we present an algorithm for an asynchronous cryptocurrency that uses proof-of-stake.
The implementation we propose uses configuration lattice agreement (CLA) and therefore is \emph{crash fault tolerant}.

\myparagraph{Cryptocurrency L-ADT.} Let us start with defining cryptocurrency as a  lattice abstract data type $(A^{\cC},B^{\cC},(\cC,\sqsubseteq^{\cC},\sqcup^{\cC}),C_0,\tau^{\cC},\delta^{\cC})$. We assume that total funds amount is constant and is equal to $M$. For simplicity, we assume that $M \in \mathbb{N}$. Set $\{1,\dots,M\}$ is denoted by $V$. We also assume that the number of unique participants of the protocol is finite and bounded by $n \in \mathbb{N}$.
We define lattice $\Lat$ $(\cC,\sqsubseteq^{\cC},\sqcup^{\cC})$ as follows: $\cC = \{ A \mid A \in \mathbb{N}_0^{n \times n }\}$, $A \sqsubseteq B \Leftrightarrow \forall i, j: a_{ij} \leq b_{ij}$, $ A \sqcup B = C$, such that $\forall i,j: c_{ij} = \textit{max}(a_{ij}, b_{ij})$. Elements $a_{ij}$  of matrix $A$ can be interpreted as ``total amount of funds transferred from account $\textit{p}_i$ to account $\textit{p}_j$''.
The initial distribution of funds is known to all and is represented by $C_0$. Formally, there is a special row for $p_0$ that makes first distribution of the funds among some participants.
%
\emph{Outputs} set  $B^{\cC} = V \cup \{ \perp\}$. 
%
\emph{Inputs} set $A^{\cC}$ contains following operations:
\begin{itemize}
    \item $\textit{transfer}(p, q, v)$ --- transfer funds in amount of $v \in V$ from account $p \in \Pi$  to account $q \in \Pi$ if the balance of $p$ allows it.
    \item $\textit{readBalance}(p)$ -- get amount of funds owned by account $p \in \Pi$.
\end{itemize}
%

%
We define transition $\tau^{\cC}$ and output $\delta^{\cC}$ functions as follows. If $a = \textit{transfer}(p, q, v)$ then $\tau^{\cC}(c, a)$ returns the new distribution matrix which is produced by applying transfer $a$ to a configuration (also a distribution matrix) $c$, else  $\tau^{\cC}(c, a) = c$.
If $a = \textit{readBalance}(p)$ then $\delta^{\cC}(c, a)$ returns the amount of funds owned by account in configuration $c$, otherwise  $\delta^{\cC}(c, a) = \perp$.
%

%
In order to complete the definition of cryptocurrency L-ADT, which is also a configuration L-ADT, we need to define the following operations: $\textit{members}(C)$, $\textit{validators}(C)$ and $\textit{quorums}(C)$. But before that, for convenience let us define function $\textit{stake}: \Pi \rightarrow V$, $stake(p) = \sum_{q=0}^{n}(A[q][p] - A[p][q])$ and the corresponding function that takes a set of processes as an argument: $\textit{stake}: 2^\Pi \rightarrow V$, $\textit{stake}(P) = \sum_{p \in P}\textit{stake}(p)$. Now we can define the required functions as follows:
\begin{itemize}
    \item $\textit{members}(C) = \{~p~|~p \in \Pi \text{ and } \exists q: C[q][p] > 0\}$
    \item $\textit{validators}(C) = \{~p~|~p \in \Pi \text{ and } \textit{stake}(p) > 0\}$
    \item $\textit{quorums}(C) = \{~Q~|~Q \subseteq \textit{validators}(C) \text{ and } stake(Q) > \dfrac{M}{2}  \}$
\end{itemize}
Members of a configuration $C$ are the processes that received funds in 
some previous (w.r.t. $\sqsubseteq^{\cC}$) configuration $C'$. The 
validators of a given configuration $C$ are the processes which have 
non-zero stake in $C$. A quorum system is a collection of sets where the 
balance of all validators of a particular quorum is more than the half of 
the total stake of the system. It is easy to see that $\forall Q, Q' \in quorums(C): Q \cap Q' \neq \emptyset$. 
Indeed, if there exist two quorums $Q$ and $Q'$ such that $Q \cap Q' = \emptyset$, 
then $\textit{stake}(Q \cup Q') = \textit{stake}(Q) + \textit{stake}(Q') > \dfrac{M}{2} + \dfrac{M}{2} > M$. 
The whole stake of the system is $M$, but we also obtain that stake of 
some part of the system is more than $M$. Contradiction.
%

%
\myparagraph{Algorithm overview.} Pseudocode of the algorithm is presented in Figure \ref{fig:poscrash}. Configuration lattice agreement as specified in Figure \ref{fig:cla}, is used as a primitive that each process holds. For now we assume that one process can be in charge of no more than one account (each replica corresponds to one and only one client). It's easy to see that presented algorithm is a special case of the one from Figure \ref{fig:ladt}.  

Once again, we assume that all operations are executed sequentially. The only place they can be interrupted is inside the CLA primitive, due to its wait condition. Functions \textit{transfer} and \textit{readBalance} correspond to the elements of input set $A^\cC$. Callback \textit{receive} is called whenever client receives a message and there is no other operation that is being executed.
We also define helper functions $sumColumnFor$ and $sumRowFor$ that calculate the respective sums for a given process identifier $r$ in order to calculate the balance of $r$. While such an operation can be performed more efficiently, we chose the presented implementation for simplicity.
%
\begin{figure}[!]
\hrule \vspace{1mm}
 {\small
\setcounter{linenumber}{0}
\begin{tabbing}
 bbbb\=bbbb\=bbbb\=bbbb\=bbbb\=bbbb\=bbbb\=bbbb \=  \kill
\textbf{Local variables:} \\
$\textit{cla}_p$ : CLA = $\textit{CLA}(C_0, \sqsubseteq^{\cC}, \sqcup^{\cC})$ \commentline{ Instance of a configuration lattice agreement } \\
$\textit{C}_p$: $\cC = C_0$  \commentline{ Local estimate of last learnt configuration } \\
\\
%
%
\textbf{fun} \textit{transfer}$(\mathit{r}: \Pi, \mathit{q}: \Pi, v: V) \rightarrow void: $\\
\nnll\label{line:poscrash:transferCheck}\> \textbf{if not} $\textit{isValidTransfer}(r, q, v)$ \textbf{then}\\
\nnll\label{line:poscrash:notValidTransfer}\>\> \textbf{return} \\
\nnll\label{line:poscrash:updateLocalConfig}\> $\textit{C}_p[r][q] \mathrel{+}= v$ \\
\nnll\label{line:poscrash:proposeConfig}\> $\textit{cla}_p.\textit{propose}(C_p)$ \\
%
\\
%
\textbf{fun} \textit{readBalance}$(\mathit{r}: \Pi) \rightarrow V: $\\
\nnll\label{line:poscrash:result}\> \textbf{return} $\textit{sumColumnFor}(r) - \textit{sumRowFor}(r)$ \\ 
%
\\
%
\textbf{callback} \textit{receive}$(m: \text{Message},\ q: \text{Sender}) \rightarrow void:$ \\
\nnll\label{line:poscrash:receive}\> $\textit{cla}_p.\textit{receive}(m,\ q)$ \\
%
\\
%
\textbf{private fun} \textit{isValidTransfer}$(r: \Pi, q: \Pi, v: V) \rightarrow Bool:$ \\
\nnll\label{line:poscrash:checkSender}\> $\textbf{if}\ r \not \eq p\ \textbf{then}$ \\
\nnll\label{line:poscrash:notThisSender}\>\> \textbf{return} \textit{false} \\
\nnll\label{line:poscrash:checkFunds}\> $\textbf{return } v \leq \textit{readBalance}(r)$ \\
%
\\
%
\textbf{private fun} \textit{sumColumnFor}$(r: \Pi) \rightarrow V:$\\
\nnll\label{line:poscrash:sumcol:initvar}\> $\textit{sum}: \text{Int} = 0$\\
\nnll\label{line:poscrash:sumcol:iterate}\> $\textbf{for}\ i\ \textbf{in}\ 0 \dots n$: \\
\nnll\label{line:poscrash:sumcol:sumplus}\>\> $\textit{sum} \mathrel{+}= C_p[i][r]$ \\
\nnll\label{line:poscrash:sumcol:return}\> $\textbf{return}\ \textit{sum}$ \\
%
\\
%
\textbf{private fun} \textit{sumRowFor}$(r: \Pi) \rightarrow V:$\\
\nnll\label{line:poscrash:sumrow:initvar}\> $\textit{sum}: \text{Int} = 0$\\
\nnll\label{line:poscrash:sumrow:iterate}\> $\textbf{for}\ i\ \textbf{in}\ 0 \dots n$: \\
\nnll\label{line:poscrash:sumrow:sumplus}\>\> $\textit{sum} \mathrel{+}= C_p[r][i]$ \\
\nnll\label{line:poscrash:sumrow:return}\> $\textbf{return}\ \textit{sum}$ \\
\end{tabbing}
}
\vspace{-1.5mm}
 \hrule
\caption{Asynchronous proof-of-stake cryptocurrency: code for process $p$.}

\label{fig:poscrash}
\end{figure}


\myparagraph{Transfer modification.} The algorithm described in Figure \ref{fig:poscrash} is very generic and there are many ways to modify it. One of the  things that is possible, is to allow transactions with multiple recipients. In order to do that we replace operation $\textit{transfer}(p, q, v)$ with $\textit{transfer}(p, \langle q_1, v_1 \rangle, \dots,\langle q_n, v_n \rangle)$, where $p$ is a sender process, $\langle q_i, v_i\rangle$ is an amount of funds $v_i$ sent to process $q_i$. Modified functions $\textit{transfer}$ and $\textit{isValidTransfer}$ are presented in Figure \ref{fig:mod}.

% \begin{figure}[!]
% \hrule \vspace{1mm}
%  {\small
% \setcounter{linenumber}{0}
% \begin{tabbing}
%  bbbb\=bbbb\=bbbb\=bbbb\=bbbb\=bbbb\=bbbb\=bbbb \=  \kill

% %
% %
% \textbf{fun} \textit{transfer}$(\mathit{r}: \Pi, \mathit{outputs}: \text{List}\langle\text{Pair}\langle\Pi,V \rangle \rangle) \rightarrow void: $\\
% \nnll\label{line:mod:transferCheck}\> \textbf{if not} $\textit{isValidTransfer}(r, outputs)$ \textbf{then}\\
% \nnll\label{line:mod:notValidTransfer}\>\> \textbf{return} \\
% \nnll\label{line:mod:updateLocalConfig}\> $\textit{outputs}.\textit{forEach}(\langle q,v \rangle \Rightarrow \textit{C}_p[r][q] \mathrel{+}= v)$ \\
% \nnll\label{line:mod:proposeConfig}\> $\textit{cla}_p.\textit{propose}(C_p)$ \\
% %
% \\
% %
% \textbf{private fun} \textit{isValidTransfer}$(r: \Pi, \mathit{outputs}: \text{List}\langle\text{Pair}\langle\Pi,V \rangle \rangle) \rightarrow Bool:$ \\
% \nnll\label{line:mod:checkSender}\> $\textbf{if}\ r \not \eq p\ \textbf{then}$ \\
% \nnll\label{line:mod:notThisSender}\>\> \textbf{return} \textit{false} \\
% \nnll\label{line:mod:checkFunds}\> $\textbf{return } \textit{outputs}.\textit{map}(\langle q,v \rangle \Rightarrow v).sum() \leq \textit{readBalance}(r)$ \\

% \end{tabbing}
% }
% \vspace{-1.5mm}
%  \hrule
% \caption{Transfer modification: code for process $p$.}

% \label{fig:mod}
% \end{figure}

==> LA-PoS/crashes/Definitions.tex <==
\myparagraph{Replicas and clients.}
Let $\Pi$ be a (possibly infinite) set of potentially participating processes. We denote them as $p_0, p_1,\dots, p_i$.
A subset of the processes, called \emph{replicas}, are used to maintain a replicated state. Any process can also act as a \emph{client}, invoking operations, but not storing anything. 
We assume that both replicas and clients are subject to crash failures: a process
\emph{fails} when it prematurely stops taking steps of its algorithm.

\myparagraph{Lattices.} \emph{Lattice}  $(\Lat, \sqsubseteq)$ is an abstract structure, where $\Lat$ 
is partially ordered by the binary relation $\sqsubseteq$ such that for any two elements $a \in \Lat$ and $b \in \Lat$ there exists $c \in \Lat$: such that $c$ is \emph{least upper bound} for set $\{a, b\}$ and $c = a \sqcup b$; also $\forall a, b \in \Lat$ $\exists\ d \in \Lat$, $d = a \sqcap b$ and $d$ is \emph{greatest lower bound} of set $\{a, b\}$. The operators $\sqcup$ and $\sqcap$ are referred as \emph{join} and  \emph{meet} respectively. Both $\sqcup$ and $\sqcap$ operators are associative, commutative, idempotent binary operators on set $\Lat$.
%
A partially ordered set in which all pairs have a join ($\sqcup$) but not necessarily a meet is called a \emph{join-semilattice}. 
%
Similarly, a partially ordered set in which any two elements have a meet ($\sqcap$) but not necessarily a join is called a \emph{meet-semilattice}. 
%

%
In this paper, we will use \emph{join-semilattice} as one of the basic types and will refer to it as a \emph{lattice}.
Intuitively, we are interested in this type, since $a \sqcup b$ can be interpreted as a \emph{merge} of two alternatively proposed operations by different replicas on some state.


\myparagraph{Abstract data types.}
%
By abstract data type ($\textit{ADT}$) we call tuple $T=(A,B,Z,z_0,\tau,\delta)$.
Here~$A$ and $B$ are countable sets called the \emph{inputs} and \emph{outputs}.  $Z$ is a countable set of abstract object \emph{states}, $z_0\in Z$ being the initial state of the object. 
The map~$\tau: Z\times A \to Z$ is the \emph{transition function}, specifying the effect of an input on the object 
state and the map~$\delta: Z\times A \to B$ is the \emph{output function}, specifying the output returned for a 
given input and object local state. 
The input represents an operation with its parameters, where (i) the operation can have a side-effect that changes 
the abstract state according to transition function $\tau$  and (ii) the operation can return values taken in the 
output $B$, which depends on the state in which it is called and the output function $\delta$ (for simplicity, we 
only consider deterministic types here.)

\myparagraph{Lattice abstract data types.}
In \emph{lattice abstract data types} ($\textit{L-ADT}$), the set of states forms a join semi-lattice 
with a partial order $\sqsubseteq^Z$. % and a join operator $\sqcup^Z$.
A lattice object is therefore defined as a tuple 
$L=(A,B,(Z,\sqsubseteq^Z,\sqcup^Z),z_0,\tau,\delta)$.\footnote{For
convenience, we explicitly specify the join operator $\sqcup^Z$ here, i.e., the least upper
bound of $\sqsubseteq^Z$.}  
%
Moreover, the transition function $\delta$ must comply 
with the partial order $\sqsubseteq^Z$, that is $\forall z,a\in Z\times A: z\sqsubseteq^Z \tau(z,a)$, and 
the composition of transitions must comply with the join operator, that is 
$\forall z\in Z,\forall a,a'\in A: \tau(\tau(z,a),a') =\tau(z,a)\sqcup^Z\tau(z,a') =\tau(\tau(z,a'),a)$.
Hence, we can say that the transition function is ``commutative''. 

\myparagraph{Composition of L-ADTs.}
%
The composition of two ADTs $T=(A,B,Z,z_0,\tau,\delta)$ and $T'=(A',B',Z',z_0',\tau',\delta')$ 
is denoted $T\times T'$ and is equal to $(A+A', B\cup B', Z\times Z',(z_0,z_0'),\tau'',\delta'')$;
where $A+A'$ denotes the disjoint union and where $\tau''$ and $\delta''$ apply, according to the domain~$A$ or $A'$ of the input, 
either $\tau$ and $\delta$ or $\tau'$ and $\delta'$ on their respecting half of the state.

\myparagraph{Configurations as L-ADTs.}
%
Let us also use the formalism of L-ADT to define a \emph{configuration L-ADT} as a tuple $(A^{\cC},B^{\cC},(\cC,\sqsubseteq^{\cC},\sqcup^{\cC}),C_0,\tau^{\cC},\delta^{\cC})$ 
with $C_0\in \cC$ the \emph{initial configuration}.  
%
For each element  $C$ of the \emph{configuration lattice} $\cC$, the input set $A$ includes following operations:
\begin{itemize}
    %
    \item $\textit{members}()$ --- an input operation, that can be considered as
    a function $\textit{members}: \cC \rightarrow 2^\Pi$, which for a given configuration
    returns a set of processes that have joined the system. More formally:
    $\delta^{\cC}(C,\textit{members}()) \subseteq \Pi$ and 
    $\forall C, C': (C \sqsubseteq C')~\Rightarrow \delta^{\cC}(C,\textit{members}()) \subseteq \delta^{\cC}(C',\textit{members}())$.
    %
    \item $\textit{validators()}$ --- an input operation, that can be considered 
    as a function  $\textit{members}: \cC \rightarrow 2^\Pi$, which for a given 
    configuration returns a set of processes that run the system (i.e. validate the messages).
    The following requirement must be met:
    $\delta^{\cC}(C,\textit{validators}()) \subseteq \delta^{\cC}(C,\textit{members}())$.
    %
    \item $\textit{quorums}()$ --- an input operation, that can be considered 
    as a function $\textit{quorums}: \cC \rightarrow 2^{2^\Pi}$, which for a given
    configuration returns a \emph{quorum system} --- a collection of subsets 
    of $\delta^{\cC}(C,\textit{validators}())$, where every two subsets have non-empty 
    intersection. Formally, $\delta^{\cC}(C, \textit{quorums}()) \subseteq 2^{\delta^{\cC}(C,\textit{validators}())}$ and 
    $\forall Q, Q' \in \delta^{\cC}(C, \textit{quorums}()): Q \cap Q' \neq \emptyset$.
\end{itemize}
With a slight abuse of notation, we will write these operations as $\textit{members}(C)$, $\textit{validators}(C)$ and $\textit{quorums}(C)$. \\
Note that any arbitrary quorum system might be used.

\myparagraph{Configuration lattice agreement.} In this paper we define a special case of reconfigurable lattice agreement (RLA)~\cite{rla}. In this instance, we don't distinguish object and configuration: object is implicitly defined by a configuration. Configuration lattice agreement operates on a lattice~($\Lat$,~$\sqsubseteq$), that is specified by a configuration L-ADT  $(A^{\cC},B^{\cC},(\cC,\sqsubseteq^{\cC},\sqcup^{\cC}),C_0,\tau^{\cC},\delta^{\cC})$. As well as reconfigurable lattice agreement, configuration lattice agreement exports a single operation \textit{propose} that takes an element of $\Lat$ as an argument and returns an element of $\Lat$ as a result.


==> LA-PoS/crashes/Model.tex <==
\myparagraph{Failure model.}
% 
When a client $p$ invokes $\textit{propose}(C)$, we say that $p$ \emph{proposes} configuration state $C$. 
%
%
We say that $p$ \emph{learns} a configuration~$C'$ if its \textit{propose} invocation returns $C'$.

We say that a configuration $C$ is \emph{potential}  
if there is a set $\{C_1,\ldots, C_k\}$ of proposed configurations such 
that~$C=C_0\sqcup^\cC(\bigsqcup^{\cC}_{i=1,\ldots,k}C_i)$ (with~$C_0$ the initial configuration).
A configuration $C$ is said to be \emph{superseded} as soon as a process learns 
a configuration $C'$ with~$C\sqsubset^{\cC} C'$.
%
At any moment of time, a configuration is \emph{active} if it is a potential but not 
yet superseded configuration.
%

%
Also, configuration $C$ is said to be \emph{surpassed} after a process learns a new configuration $C'$ such that $C\sqsubset^{\cC} C'$  and $\textit{members}(C) \subset \textit{members}(C')$.
%

%
We say that a replica $r$ is \emph{active} when it is a member of 
an active configuration $C$, i.e., $r\in \textit{member}(C)$. 
%The intuition here is that a replica can be removed from the system as
%soon as it not active any longer.  
A replica is \emph{correct} if, from some point on, it is forever
active and not failed.
A \emph{client} is correct if it does not fail while executing a
\textit{propose} operation.
%

A configuration $C$ is \emph{available} if some set of replicas in $\textit{quorums}(C)$
contains only correct processes. \\
%
 \myparagraph{Correctness properties.}
 %
 In this paper we assume that following \textbf{availability} property is always true: any potential configuration that is \textit{never surpassed} is available. Algorithm that is presented in the next section satisfies following properties:

\begin{itemize}
    \item \textbf{Consistency.} The learnt values are totally ordered by $\sqsubseteq$.
    \item \textbf{Validity.} If $\textit{propose}(c)$ returns a value $c'$ then $c'$ is a join of some proposed values including $c$ and all learnt values before the function invocation.
    \item \textbf{CLA-Liveness.} In executions where the number of unique members is limited by some $n \in \mathbb{N}$, every $propose$ operation invoked by a correct process eventually returns. More precisely, $\exists n \in \mathbb{N},\ \forall C \in \cC: \lvert\textit{members}(C)\rvert \leq n$.
\end{itemize}

It has been shown that asynchronous runs with infinitely many 
reconfigurations don't ensure wait-freedom~\cite{r-liveness}.
In our case, configuration not only holds a set of current replicas, but also some 
complementary object (e.g. weights distribution when weighted quorum system is considered).
In order to ensure the system's liveness we require the number of processes that join the system 
to be finite, however any other additional information associated with replicas can change infinitely. 
In practice, this restriction boils down to assuming sufficiently 
long periods of time when no new participants join the system.
%



==> LA-PoS/crashes/OptimMes.tex <==
\textbf{IN PROGRESS}

It might be noticed that in proposed algorithms processes always send 
messages that contain configuration objects. However configuration can be 
sufficiently large or, what's even worse, unbounded in size: a common 
example of such a configuration object is add-only set. It can lead to a 
problem in applying algorithm in practice, as throughput capacity of 
network channels is limited.
%
%
In order to work around this problem, we can modify presented algorithms.
Instead of sending a whole configuration $c_p$ (local commit estimate), every process $p$ only sends a set of \emph{deltas} to
other process that uniquely identify how its local commit estimate has 
changed since last message. Basically, we need process $p$ to send only some \emph{delta} that represents part of 
learnt configuration that has been changed. Also, for every $q$ it locally stores \emph{deltas} that have not yet been sent to the process $q$.

We define an \emph{``expansion''} function $\textit{exp}: \Delta \rightarrow Z$ over a lattice $\Lat\ (Z, \sqsubseteq^Z, \sqcup^Z)$  that transforms given $\delta \in \Delta$ to some element of a lattice $z \in Z$. For simplicity, we also define function with the same name $\textit{exp}$ that for a given set $\textit{D} \subseteq \Delta$ returns a set of elements from lattice $\Lat$: $\textit{exp}(D) = \{\textit{exp}(\delta) ~|~\delta \in D\}$. We only need this function in order to ``apply'' delta $\delta$ to an element of a lattice.

Let's take a look at some lattices and apply our idea to them: 
\begin{itemize}
    \item \textbf{Add-only set.} By delta we mean an element that is added to added to a set. Expansion function is defined as follows: $\textit{exp}(\delta) = \{\delta\}.$
    \item \textbf{Max matrix.} In the max matrix lattice (that we used in cryptocurrency L-ADT) delta is considered as a tuple $\delta = \langle i, j, v \rangle$, expansion function is $\textit{exp}(\langle i, j, v \rangle) = A$, where $A[i][j] = v$ and $\forall i', j', i' \neq i, j' \neq j: A[i'][j'] = 0$.
\end{itemize}



\myparagraph{Overview.} TODO

%
\begin{figure}[!]
\hrule \vspace{1mm}
 {\small
\setcounter{linenumber}{0}
\begin{tabbing}
 bbbb\=bbbb\=bbbb\=bbbb\=bbbb\=bbbb\=bbbb\=bbbb \=  \kill
\textbf{Local variables:} \\
$\textit{seq}_p : \text{Int} = 0$\ \ \ \ \commentline{The number of issued requests}\\
$c_p : \cC$ = $C_0$\ \ \ \ \ \ \   \commentline{The last learnt configuration}\\
$T_p : \text{Set}\langle \Delta \rangle$ = $\emptyset$\commentline{The set of proposed deltas}\\
$ToSend: \text{Array}\langle \text{Set}\langle\Delta\rangle \rangle = [\emptyset] \cdot n$ \commentline{$\forall q$ set of deltas that are to be sent to process $q$ }\\
\\
%
%
\textbf{fun} \textit{propose}$(\delta: \Delta) \rightarrow \cC: $\\
\nnll\label{line:clad:initState}\> $\textit{updateState}(\emptyset,\{\delta\})$\\
\nnll\label{line:clad:while}\> \textbf{while} \textit{true} \textbf{do}\\
\nnll\label{line:clad:seqNum}\>\> $\textit{seq}_p = \textit{seq}_p+1$\\
\nnll\label{line:clad:refCommit}\>\> $\mathit{oldCommit} =  c_p$.\textit{copy}$()$ \\
\nnll\label{line:clad:refCandidates}\>\> $\mathit{oldCandidates} = T_p$.\textit{copy}$()$ \\
\nnll\label{line:clad:queriedConfs}\>\> $V = \{\bigsqcup^\cC (\{c_p\}\cup \mathit{exp}(S))~|~S\subseteq T_p\}$\commentline{Queried configurations}\\
\nnll\label{line:clad:iterate}\>\> $\textbf{for } q\ \textbf{in}\ 0...n\ \textbf{do}$\\
\nnll\label{line:clad:send_p}\>\>\> $\mathit{send}(\langle(REQ, seq_p), (ToSend[q], T_p) \rangle,\ q)$\\
\nnll\label{line:clad:wait}\>\> \textbf{wait until} $\mathit{oldCommit} \neq c_p$ \textbf{or} 
$\forall u \in V$, received responses of the type  \\
\>\>\>\>\>  $\langle (\textit{RESP},\textit{seq}_p),\_ \rangle$ from some $Q\in\textit{quorums}(u)$\\
\nnll\label{line:clad:noInterrupt}\>\> \textbf{if}  $\mathit{oldCommit}=c_p$ \textbf{and} $\mathit{oldCandidates} = T_p$ \textbf{then}  \commentline{Stable configurations}\\
\nnll\label{line:clad:iterate2}\>\>\> $\textbf{for } q\ \textbf{in}\ 0...n\ \textbf{do}$\\
\nnll\label{line:clad:commit}\>\>\>\> $\mathit{send}(\langle \textit{COMMIT}, (ToSend[q] \cup T_p, \emptyset)\rangle,\ q)$ \\
\nnll\label{line:clad:clearDeltas}\>\>\>\> $ToSend[q].clear()$ \\
\nnll\label{line:clad:return}\>\>\> \textbf{return} $(\bigsqcup^\cC (\{c_p\}\cup \mathit{exp}(T_p)))$\\ 
\nnll\label{line:clad:otherCommit}\>\> \textbf{if} $\mathit{exp}(\delta) \sqsubseteq 
c_p $ \textbf{then} \\
\nnll\label{line:clad:otherCommitReturn}\>\>\> \textbf{return} $c_p$ \\
\\
%
%
\textbf{private fun} \textit{updateState}$(D: \text{Set}\langle \Delta \rangle,\ S_C: \text{Set}\langle \Delta \rangle) \rightarrow \textit{void}:$ \\
\nnll\label{line:clad:newCommit}\> $c_p = c_p \sqcup \mathit{exp}(D)$\\
\nnll\label{line:clad:newConfs}\> $T_p = \{u\in (T_p\cup S_C)~|~c_p \sqcup \mathit{exp}(u) \not\sqsubseteq^\cC c_p \}$ \\
\\
%
%
\textbf{callback} \textit{receive}$(\langle \textit{msgType},\ \textit{msgContent} \rangle: \text{Message},\ q: \text{Sender}) \rightarrow void:$ \\
\nnll\label{line:clad:mergeReceived}\> $updateState(\textit{msgContent})$ \\
\nnll\label{line:clad:ifCommit}\> \textbf{if} $\textit{msgType}=\textit{COMMIT} $ \textbf{then} \\
\nnll\label{line:clad:addToSend}\>\> $\textbf{for } q\ \textbf{in}\ 0...n\ \textit{ToSend}[q].\textit{add}(\textit{msgContent}.\delta)$ \\
\nnll\label{line:clad:sendback}\> \textbf{if} $\textit{msgType}=(\textit{REQ},\textit{seq}) $ \textbf{then} \\
\nnll\label{line:clad:sendback2}\>\>  \textit{send}$(\langle (\textit{RESP},\textit{seq}),(ToSend[q],T_p)\rangle,~q)$ \\
\nnll\label{line:clad:clearAfterSendBack}\>\> $ToSend[q].clear()$ \\
\end{tabbing}
}
\vspace{-1.5mm}
 \hrule
\caption{Universal reconfiguration construction with delta optimization: code for process $p$.}

\label{fig:clad}
\end{figure}


%
\begin{figure}[!]
\hrule \vspace{1mm}
 {\small
\setcounter{linenumber}{0}
\begin{tabbing}
 bbbb\=bbbb\=bbbb\=bbbb\=bbbb\=bbbb\=bbbb\=bbbb \=  \kill
\textbf{Local variables:} \\
$\textit{cla}_p$ : CLA = $\textit{CLA}(C_0, \sqsubseteq^{\cC}, \sqcup^{\cC})$ \commentline{ Instance of a configuration lattice agreement } \\
$\textit{C}_p$: $\cC = C_0$  \commentline{ Local estimate of last learnt configuration } \\
\\
%
%
\textbf{fun} \textit{transfer}$(\mathit{r}: \Pi, \mathit{q}: \Pi, v: V) \rightarrow void: $\\
\nnll\label{line:poscrashd:transferCheck}\> \textbf{if not} $\textit{isValidTransfer}(r, q, v)$ \textbf{then}\\
\nnll\label{line:poscrashd:notValidTransfer}\>\> \textbf{return} \\
\nnll\label{line:poscrashd:updateLocalConfig}\> $\textit{C}_p[r][q] \mathrel{+}= v$ \\
\nnll\label{line:poscrashd:proposeConfig}\> $\textit{cla}_p.\textit{propose}(\langle r, q, v\rangle)$ \\
%
\\
%
\textbf{fun} \textit{readBalance}$(\mathit{r}: \Pi) \rightarrow V: $\\
\nnll\label{line:poscrashd:result}\> \textbf{return} $\textit{sumColumnFor}(r) - \textit{sumRowFor}(r)$ \\ 
%
\\
%
\textbf{callback} \textit{receive}$(m: \text{Message},\ q: \text{Sender}) \rightarrow void:$ \\
\nnll\label{line:poscrashd:receive}\> $\textit{cla}_p.\textit{receive}(m,\ q)$ \\
%
\\
%
\textbf{private fun} \textit{isValidTransfer}$(r: \Pi, q: \Pi, v: V) \rightarrow Bool:$ \\
\nnll\label{line:poscrashd:checkSender}\> $\textbf{if}\ r \not \eq p\ \textbf{then}$ \\
\nnll\label{line:poscrashd:notThisSender}\>\> \textbf{return} \textit{false} \\
\nnll\label{line:poscrashd:checkFunds}\> $\textbf{return } v \leq \textit{readBalance}(r)$ \\
%
\\
%
\textbf{private fun} \textit{sumColumnFor}$(r: \Pi) \rightarrow V:$\\
\nnll\label{line:poscrashd:sumcol:initvar}\> $\textit{sum}: \text{Int} = 0$\\
\nnll\label{line:poscrashd:sumcol:iterate}\> $\textbf{for}\ i\ \textbf{in}\ 0 \dots n$: \\
\nnll\label{line:poscrashd:sumcol:sumplus}\>\> $\textit{sum} \mathrel{+}= C_p[i][r]$ \\
\nnll\label{line:poscrashd:sumcol:return}\> $\textbf{return}\ \textit{sum}$ \\
%
\\
%
\textbf{private fun} \textit{sumRowFor}$(r: \Pi) \rightarrow V:$\\
\nnll\label{line:poscrashd:sumrow:initvar}\> $\textit{sum}: \text{Int} = 0$\\
\nnll\label{line:poscrashd:sumrow:iterate}\> $\textbf{for}\ i\ \textbf{in}\ 0 \dots n$: \\
\nnll\label{line:poscrashd:sumrow:sumplus}\>\> $\textit{sum} \mathrel{+}= C_p[r][i]$ \\
\nnll\label{line:poscrashd:sumrow:return}\> $\textbf{return}\ \textit{sum}$ \\
\end{tabbing}
}
\vspace{-1.5mm}
 \hrule
\caption{Asynchronous proof-of-stake cryptocurrency with delta optimization: code for process $p$.}

\label{fig:poscrashd}
\end{figure}

==> LA-PoS/draft.tex <==
% \begin{lemma}
% \label{lm:tvpprogres}
% In every execution with at least one invocation of $\textit{TxValObj}.\text{Validate}(tx,\sigma_{tx})$ operation (line \ref{line:posmain:validate}) by a forever-correct process, 
% some forever-correct process $p$ returns a verifiable set of transactions (along with corresponding certificate) from $\textit{TxValObj}.\text{Validate}(tx',\sigma_{tx}')$ (line \ref{line:posmain:validate}). 
% \end{lemma}
% \begin{proof}
% We will prove this fact by contradiction. 
% Let us assume that there is no such forever-correct process, that returns a verifiable set of transactions (along with corresponding certificate) from $\textit{TxValObj}.\text{Validate}(tx,\sigma_{tx})$ at line \ref{line:posmain:validate}.
% In this case, no forever-correct process updates its local history (the only way to obtain a verifiable history is to pass through the entire $\code{Transfer}(..)$ operation, including $\textit{TxValObj}.\text{Validate}(tx,\sigma_{tx})$), then $\textit{history} = \{C_{init}\}$ and $C_{inst} = C_{cur} = C_{init}$. 
% At the same time, the number of the system members is bounded from above by some $n$, the number of valid transactions each member can submit is also limited, as the whole stake of the system is limited and no new transactions are added to configuration.
% Hence, at some point of time all forever-correct processes will have the same set \textit{validTxs}. 
% It means that eventually some forever-correct process $p$ will be able to collect required signatures and, thus, some verifiable transaction set will be returned. 
% We came to a contradiction, what means that our assumption was wrong. 
% Therefore, the statement of the lemma is proved.
% \end{proof}

% \begin{lemma}
% \label{lm:systvprogres}
% If some forever-correct process invoked $\textit{TxValObj}.\text{Validate}(tx,\sigma_{tx})$ operation (line~\ref{line:posmain:validate}) at some moment of time $t$,
% then some forever-correct process $p$ returns a verifiable set of transactions (along with corresponding certificate) from $\textit{TxValObj}.\text{Validate}(tx',\sigma_{tx}')$  (line~\ref{line:posmain:validate}) at some point of time $t'$ ($t' \ge t$).
% \end{lemma}
% \begin{proof}
% By applying proof of the Lemma \ref{lm:tvpprogres} inductively we obtain the desired.
% \end{proof}


% \begin{lemma}
% \label{lm:tvpliveness}
% Every valid transaction $tx$ issued by a forever-correct process is guaranteed to be a part of some verifiable transaction set returned by a forever correct process from $\textit{TxValObj}.\text{Validate}(tx',\sigma_{tx}')$ (line~\ref{line:posmain:validate}).
% \end{lemma}
% \begin{proof}
% As well as for Lemma~\ref{lm:tvpprogres}, in order to prove this fact we use indirect proof technique.
% We assume that there is a transaction $tx$ issued by a forever-correct process, that doesn't conflict with any other ever-issued transaction, and that is never included in any verifiable transaction set returned from  $\textit{TxValObj}.\text{Validate}(tx',\sigma_{tx}')$ by a forever-correct process.
% As the number of the system members is limited by some $n$, then eventually every forever-correct process will add this transaction $tx$ to its local set $\textit{seenTxs}$. 
% At a later point of time one of the forever correct processes $p$ will collect the validation responses for a set $\textit{sentTxs} \subseteq \textit{seenTxs}$. 
% As $tx$ is in  $\textit{seenTxs}$ and $tx$ doesn't conflict with any other ever-issued transaction, then $tx$ will also be included in $\textit{sentTxs}$. After acknowledgments are gathered,  $p$ returns a verifiable set of transactions $txs$ from $\textit{TxValObj}.\text{Validate}(tx',\sigma_{tx}')$ with corresponding certificate.
% It's easy to see that $tx$ will be included in $txs$ (not only in $\textit{sentTxs}$), as no other process is able to provide a "proof of conflict'' (a transaction that conflicts with $tx$), due to the fact that the sender signature cannot be forged.
% The existence of such a forever-correct process $p$ follows from the Lemma~\ref{lm:systvprogres}.
% \end{proof}


% \begin{lemma}
% \label{lm:configlaprogres}
% In every execution with at least one invocation of $\textit{ConfigLA}.\text{Propose}(txs,\sigma_{txs})$ operation (line~\ref{line:posmain:configpropose}) by a forever correct process,
% some forever correct process $p$ returns a verifiable value (along with corresponding certificate) from $\textit{ConfigLA}.\text{Propose}(txs',\sigma_{txs}')$ (line~\ref{line:posmain:configpropose}). 
% \end{lemma}

% \begin{proof}
% The proof is carried out in the same way as in Lemma \ref{lm:tvpprogres}.
% \end{proof}


% \begin{lemma}
% \label{lm:sysconfiglaprogres}
% If some forever-correct process invoked $\textit{ConfigLA}.\text{Propose}(txs,\sigma_{txs})$ operation (at line~\ref{line:posmain:configpropose}) at some moment of time $t$,
% then some forever-correct process $p$ returns a verifiable set of transactions (along with corresponding certificate) from $\textit{ConfigLA}.\text{Propose}(trs',\sigma_{trs}')$ (at line \ref{line:posmain:configpropose}) at some point of time $t'$ ($t' \ge t$).
% \end{lemma}

% \begin{proof}
% By applying proof of the Lemma \ref{lm:configlaprogres} inductively we obtain the desired.
% \end{proof}


% \begin{lemma}
% \label{lm:configlaliveness}
% If a verifiable input value $txs$ is submitted to \textit{ConfigLA} (line \ref{line:posmain:configpropose}) by some forever-correct process, then eventually some forever-correct process $p$ returns a verifiable output value $T$ with corresponding certificate from $\textit{ConfigLA}.\text{Propose}(txs',\sigma_{txs}')$ (line~\ref{line:posmain:configpropose}), such that $txs \sqsubseteq T$.
% \end{lemma}

% \begin{proof}
% We prove this fact by contradiction.
% We assume that there is a verifiable input value $txs$ submitted by a forever-correct process to \textit{ConfigLA}, and no forever-correct process returns a verifiable output value $T$ from \textit{ConfigLA} such that $txs \sqsubseteq T$.
% As number of the system members is limited by some $n$, then eventually every forever correct process will add verifiable input value $txs$ to its local set $\textit{values}$. 
% At a later point of time, when sets $\textit{values}$ of all forever-correct processes become identical,  one of the forever correct processes $p$ will collect required signatures and return a verifiable output value $T = \bigsqcup \textit{values}$. As $trs \in \textit{values}$, $trs \sqsubseteq T$.
% The existence of such a forever-correct process $p$ follows from the Lemma~\ref{lm:sysconfiglaprogres}.
% \end{proof}

% \begin{lemma}
% \label{lm:historylaliveness}
% Lemmas, equivalent to Lemma \ref{lm:configlaprogres}, Lemma \ref{lm:sysconfiglaprogres}, Lemma \ref{lm:configlaliveness}, can be formulated for \textit{HistoryLA} and proved in the same way. 
% \end{lemma}
% \begin{proof}
% Indeed, \textit{ConfigLA} and \textit{HistoryLA} have the same implementation. The only difference between them is the type used as lattice. Hence, the proofs can be reused.
% \end{proof}

==> LA-PoS/related_work.tex <==

The most prevalent cryptocurrencies today do not use a traditional Byzantine fault tolerance algorithm but rely on the proof-of-work approach that requires users to compete against each other for the right to append the next block to the chain by solving a computationally complex cryptographic problem first and a reward system for doing so. E.g., in Bitcoin~\citep{bitcoin} and 
Ethereum~\citep{ethereum} the hash of a block must start with many zeros and the longest chain of blocks is considered authoritative. The goal of this approach is to ensure that computational power is used to extend the current longest chain with valid blocks and creating many pseudonyms is not advantageous. However, the possibility of two chains of blocks (forks) being extended is problematic and leads to an unfortunate trade-off between the time a transaction can be considered confirmed (by several blocks extending the chain with the transaction) and the security guarantees required by applications. Moreover, the success of cryptocurrencies has led to high transaction fees, an enormous energy consumption and the use of expensive specialized hardware to solve the cryptographic puzzles and as a consequence the system is maintained by a small number of powerful mining pools instead of a vast number of truly decentralized machines.

To mitigate these problems, relying on the users' stake instead of their computational power (proof-of-stake) has been suggested. In PoS approaches, users can influence the evolution of the cryptocurrency in proportion to the amount of currency they own. The advantages over PoW include better energy efficiency, reduced hardware requirements and thus a more decentralized setup with more nodes maintaining the system. PoS also enables systems to punish users if they misbehave, e.g., by losing a part of their stake if they are offline and do not process transactions or if they deliberately violate the protocol, e.g., by confirming invalid transactions with their signature.

In the next version of Ethereum ~\citep{ethereum_pos}, users can stake a minimum amount to become a validator -- a node responsible for checking transactions and creating new blocks. The protocol will repeatedly choose random committees of 128 validator nodes from the set of validators, thus balancing the load and mitigating adaptive corruption attacks.
In Algorand~\citep{gilad2017algorand} all users can contribute by taking part in a cryptographic lottery process to be randomly and secretly, yet provably elected to propose blocks and vote on block proposals. The probability of being chosen and the weight of the votes is proportional to the assets owned by the user. To avoid adaptive corruption, the election proof is only valid for one action, i.e., as soon as others learn about a user's right to propose or vote it is too late to start to try and influence them.
Ouroboros~\citep{ouroboros17}, another PoS protocol, on the other hand, relies on the assumption that most users are incorruptible by the adversary for a significant epoch (such as a day).

The fact that these PoS approaches are based on consensus ensures that all users have the view of the distribution of assets among the users for each block height, which simplifies the protocols and proofs considerably.

Most cryptocurrencies enforce a total order over the transactions by batching them in blocks and running consensus protocol to decide which block to attach to the chain next. This has the advantage that blocks can contain any instructions on how to change the state maintained by the replica (in other words implementing a general replicated state machine via \emph{smart contracts}), the drawbacks of the FLP result~\citep{FLP85} regarding consensus solutions apply, namely the fact that no deterministic implementation for an asynchronous system can exist.


It has been shown~\citep{Gup16,at2-cons} that consensus is not necessary for implementing asset transfer, as it suffices to order the outgoing transactions for each participant separately and~\citep{astro-dsn} demonstrated how a fully asynchronous system based on reliable broadcast algorithms can implement a (sharded) cryptocurrency in a simpler, more efficient and more robust fashion that consensus-based solutions. In their design, a static set of replica processes the transactions, i.e., the protocol adheres to the \emph{permissioned} model.
%
To overcome this short-coming, \citep{byz-bcast} presents a reliable broadcast protocol to allow replicas to join or leave the system without requiring consensus.

More general work in this direction is based on generalized lattice agreement. Recent results show how to represent the dynamic membership in a \emph{lattice order}~\citep{rla} and propose a protocol properly reconcile different opinions on which members are active in an asynchronous fashion for crash-stop failures, extended to the Byzantine cased in~\citep{bla}. In particular, forward-secure digital signatures ensure that slow clients cannot be tricked by superseded and possibly compromised configurations to consider stale data up to date and the protocol also prevents Byzantine clients to executed a denial of service by flooding the system with reconfiguration requests. Our results build on top of these results and shows how to adapt them to allow for weighted reconfigurable quorums and implement a cryptocurrency.

A fully asynchronous and consensus-free PoS protocol for a cryptocurrency was proposed in ~\citep{abc-tr}. Instead of blocks with transactions forming a chain, transactions with multiple inputs and outputs form a directed acyclic graph. Each transaction specifies a validator (may be the owner of one of inputs). A validator broadcasts a signed ack messages containing references to its previous ack message and to a set of valid non-conflicting transactions it received. 
A transaction is considered confirmed if it has been acknowledged by validators with a total sum of delegated stake of more than 2/3 of the total amount of funds in the system. A validator $v$'s delegated stake in a set of acks for a set of transactions and their transitive closure is defined recursively to be equal to the sum of the output values of confirmed transactions delegated to $v$ which have not been used as inputs in the set of transactions and their transitive closure. 
Unfortunately, the proofs implicitly rely on a static adversary, in the sense that the members to be corrupted must be chosen at the beginning.
